Quizbowl: The Case for Incremental Question Answering

Scholastic trivia competitions test knowledge and intelligence through mastery of question answering. Modern question answering benchmarks are one variant of the Turing test. Specifically, answering a set of questions as well as a human is a minimum bar towards demonstrating human-like intelligence. This paper makes the case that the format of one competition -- where participants can answer in the middle of hearing a question (incremental) -- better differentiates the skill between (human or machine) players. Additionally, merging a sequential decision-making sub-task with question answering (QA) provides a good setting for research in model calibration and opponent modeling. Thus, embedded in this task are three machine learning challenges: (1) factoid QA over thousands of Wikipedia-like answers, (2) calibration of the QA model's confidence scores, and (3) sequential decision-making that incorporates knowledge of the QA model, its calibration, and what the opponent may do. We make two contributions: (1) collecting and curating a large factoid QA dataset and an accompanying gameplay dataset, and (2) developing a model that addresses these three machine learning challenges. In addition to offline evaluation, we pitted our model against some of the most accomplished trivia players in the world in a series of exhibition matches spanning several years. Throughout this paper, we show that collaborations with the vibrant trivia community have contributed to the quality of our dataset, spawned new research directions, and doubled as an exciting way to engage the public with research in machine learning and natural language processing.

==> 2021_jmlr_qanta/sections/35-syndiv.tex <==
\subsubsection{Syntactic Diversity}
\label{sec:syn-div}

This section argues that \qb{} is more syntactically diverse than other factoid
question answering datasets.
%
Syntactic diversity is desirable because
different, yet equivalent, framings of the same question should be handled
equally well by trained models, but are often
not~\citep{IyyerSCPN2018}.
%
Additionally, diversity discourages models from building (invalid) connections
between specific syntactic structures (artifacts) and specific
answers~\citep{Gururangan2018AnnotationAI,feng2018rawr}.

We use constituency parses~\citep{corenlp, corenlp_parse} to capture
the syntax of sentences:\footnote{We use the shift-reduce parser in
    version 3.9.1 of Stanford CoreNLP.  We exclude terminals; otherwise
    every unique question would trivially be a unique parse} the more
distinct parse trees, the more syntactic diversity.
%
However, diversity is more important at the top of the tree; there is
a bigger difference between ``who was the last whig president'' and
``which whig was the last to hold the presidency'' than between
``which whig was the last to hold the presidency'' and ``which whig
from New York was the last to hold the presidency'' (Figure~\ref{fig:parses}).
%
To capture this distinction we compare the number of unique parses
depth~$d$ in the parse tree.
%
If a dataset is diverse, it should show diversity across a wide range
of maximum tree depths; datasets generated from templates will show
little diversity, particularly at shallow depths.

\begin{figure}[t] % TODO: Font still isn't right size
    \centering
    \includegraphics[width=\linewidth]{jmlr-parse-tree}
    \caption{Here we show the constituency parse trees for two similar sentences.
        The syntactic structure of the sentences is identical until depth $d=4$. In our
        analysis we compute the number of unique parses as a function of $d$, ranging
        from one to ten, on several  \abr{qa} datasets.}
    \label{fig:parses}
\end{figure}

\begin{figure*}[ht]
    \centering \includegraphics[width=1.0\textwidth]{syn_div_plot}
    \captionof{figure}{The syntactic diversity of \abr{qa} datasets
        measured through their constituency parses.  More diverse datasets
        should have more total unique parse trees (bottom plot), and
        unique parses per instance (top plot). To
        avoid minor variations deeper in parse trees from impacting
        results too heavily we plot counts and averages for a range of
        constituency tree truncation depths. At each truncation depth, we
        prune any part of the tree which is deeper than the specified
        depth before computing uniqueness of parses. Consider
        $S\rightarrow \text{NP VP}$. Under truncation depth one this
        becomes $S$ while under truncation depth two it remains the same.}
    \label{fig:syn-div}
\end{figure*}


Both competitive trivia datasets---\qb{} and Jeopardy!---are more
diverse on average, and \qb{} has significantly more unique
constituency parses (Figure~\ref{fig:syn-div}).
%
These results are consistent across all depths.
%
This confirms that questions authored by crowd workers are less
diverse than those authored by experts/enthusiasts (\qb{}, TriviaQA,
and Jeopardy!).

However, counting trees is a blunt instrument (and could bias toward
our larger dataset's long tail).
Instead, we first assume each dataset is generated by a distribution over syntax represented by context-free grammars~\citep{chomsky-56}.
Next, we estimate a probabilistic context-free grammar (\abr{pcfg}) for each dataset as proposed by~\citet{booth69}.
Finally, we compute the entropy of \abr{pcfg} and compare this value across datasets.

Following the process and notation of~\citet{Jurafsky2009}, we use the constituency parses of the questions to build a \abr{pcfg} of non-terminal symbols $N$, terminal symbols $\Sigma$, rules $R$ of the form $A\rightarrow\beta\ [p]$, and a start symbol $S$.
In this notation, $A$ is a non-terminal, $\beta$ is a string of symbols from the infinite set of strings $(\Sigma\cup N)*$, and $p$ represents the probability $P(A\rightarrow\beta | A)$.
We estimate the probability
\begin{equation}
    P(A\rightarrow\beta | A)=\frac{Count(A \rightarrow \beta)}{Count(A)}
\end{equation}
of each rule by counting the frequency of each transition in the parses for each dataset.
Lastly, we compute the entropy of the \abr{pcfg}
\begin{align}
    \h{}{N, S, R} & =\h{}{P(A)P(A\rightarrow\beta | A)}                                                              \\
                  & =-\sum_{A\rightarrow\beta\in R} P(A)P(A\rightarrow \beta | A)\log P(A) P(A\rightarrow \beta | A)
\end{align}
by normalizing the probability of each rule by the frequency of the non-terminal $A$.

The entropy of the \textsc{pcfg} for each dataset is in
Table~\ref{table:entropy}.
%
From this comparison we reach conclusions similar to those from
Figure~\ref{fig:syn-div}; the \qanta{} dataset has more diverse and
sophisticated examples than datasets crowdsourced online.
%
This is not surprising as questions from the \qanta{} datasets,
TriviaQA, and SearchQA (Jeopardy!) are often written by domain
experts, and sometimes even professional writers.


\begin{table}
    \centering
    \begin{tabular}{ l r}
        \toprule
        Dataset                   & \textsc{pcfg} Entropy \\
        \midrule
        \triviaqa{}               & 5.64                  \\
        \qanta{} 2018 (This Work) & 5.48                  \\
        \searchqa{}               & 5.41                  \\
        \squad{} 1.0              & 5.30                  \\
        \simplequestions{}        & 4.53                  \\
        \bottomrule
    \end{tabular}
    \caption{}
    \label{table:entropy}
\end{table}

==> 2021_jmlr_qanta/sections/leftover.tex <==

% \jbgcomment{Talk about time component of optimal buzzer}
%
% We consider the outcomes of action $A(t) \in {0,1}$ where $0$ means waiting and
% $1$ means buzzing. We use $C(t) \in {0,1}$ to indicate if the guesser is correct
% at time $t$. We use $t_g$ to indicate the time when the guesser is correct for
% the first time, so $t_g = \min t$ s.t. $C(t) = 1$, we define $t_g=-1$ when the
% guesser is never correct.
%
% The outcome of action $A(t)$ is divided in to the following categories:
%
% \begin{itemize}
%     \item Buzz wrong: $t < t_g$ but $A(t) = 1$
%     \item Buzz correct: $A(t) = 1$ and $C(t) = 1$
%     \item Buzz miss: $t > t_g$ and $A(t) = 1$ but $C(t) = 0$
%     \item Wait correct: $t < t_g$ and $A(t) = 0$
%     \item Wait wrong: $t > t_g$ and $C(t) = 1$ but $A(t) = 0$
%     \item Buzz impossible: $t_g = -1$ but $A(t) = 1$
%     \item Wait impossible: $t_g = -1$ and $A(t) = 0$
% \end{itemize}
%
% The outcome can be summarized in a different way:
%
% \begin{itemize}
%     \item Guesser is correct at one point $t_g > 0$
%         \begin{itemize}
%             \item Before guesser is correct $t < t_g$
%                 \begin{itemize}
%                     \item Wait $\rightarrow$ correct
%                     \item Buzz $\rightarrow$ wrong
%                 \end{itemize}
%             \item After guesser is correct $t >= t_g$
%                 \begin{itemize}
%                     \item Wait $\rightarrow$ wrong
%                     \item Buzz $\rightarrow$ correct or miss
%                 \end{itemize}
%         \end{itemize}
%     \item Guesser is never correct $t_g = -1$
%         \begin{itemize}
%             \item Buzz $\rightarrow$ wrong
%             \item Wait $\rightarrow$ correct
%         \end{itemize}
% \end{itemize}

% \paragraph{Against the Simulated Human Players}
%
% \jbgcomment{This should either be expanded or cut substantially}
%
% As described in Section~\ref{Refer protobowl data section}, we
% collected data of human playing QuizBowl from Protobowl. We evaluated
% our system against the human players by simulating games using these
% data.
%
% \jbgcomment{Why are we recording this information; what's the topic
%   sentence?}
%
% We keep record of several statistics during the simulated games.  We
% are curious if the classifier buzzer would work playing against an
% opponent, as there is no opponent modeling in the buzzer. We first
% classify the game outcomes in two categories: \textit{possible} games
% and \textit{impossible} games.  \textit{Possible} means either the
% guesser gets it correct before the opponent buzzes, or the opponent
% gives a wrong answer. In these games the guesser has done a good job
% and it takes the buzzer to buzz smartly and beat the opponent.  On the
% other hand \textit{impossible} means the opponent answers correctly
% before the guesser gets it correct, in which case there is nothing
% that the buzzer can do, other than not buzzing at all.
%
% \begin{itemize}
%     \item Buzzing position
%         \begin{itemize}
%             \item Before opponent
%             \item After opponent
%         \end{itemize}
%     \item Winning method
%         \begin{itemize}
%             \item Buzz and answer before the opponent buzzes
%             \item After opponent buzzes and gives a wrong answer
%         \end{itemize}
%     \item Buzzer
%         \begin{itemize}
%             \item \textit{Possible} games: rush or delay
%             \item \textit{Impossible} games: rush or delay
%         \end{itemize}
% \end{itemize}
%
% The simulated human player is at a slight disadvantage. When machine
% buzzes and gives a wrong answer, the opponent should be able to answer
% based on the whole question. But since we only have the answer given
% by human players when they buzz, we don't know what they would have
% answered if they see the whole question.
%
% Besides the statistics mentioned above, we also calculate the scores
% against the opponent. We want to know the average score against
% different levels of plays.  We sort the players by the number of
% games they played as a metric of how good they are at
% QuizBowl. \fscomment{probably should use their score against other
%   human players}
